A Case for a Programmable Edge Storage Middleware

Edge computing is a fast-growing computing paradigm where data is processed at the local site where it is generated, close to the end-devices. This can benefit a set of disruptive applications like autonomous driving, augmented reality, and collaborative machine learning, which produce incredible amounts of data that need to be shared, processed and stored at the edge to meet low latency requirements. However, edge storage poses new challenges due to the scarcity and heterogeneity of edge infrastructures and the diversity of edge applications. In particular, edge applications may impose conflicting constraints and optimizations that are hard to be reconciled on the limited, hard-to-scale edge resources. In this vision paper we argue that a new middleware for constrained edge resources is needed, providing a unified storage service for diverse edge applications. We identify programmability as a critical feature that should be leveraged to optimize the resource sharing while delivering the specialization needed for edge applications. Following this line, we make a case for eBPF and present the design for Griffin - a flexible, lightweight programmable edge storage middleware powered by eBPF.

==> 2_edge_landscape.tex <==
Before delving into why the edge needs a \textit{programmable storage middleware}, 
a valid first question to ask is whether the edge needs a storage service. 


The majority of edge-related benefits come from having timely, in-field, 
low-latency access to data~\cite{2012-mcc-edge-vision,2017-hotcloud-keynote-satya-edge}.
In cloud datacenters typically a shared, reliable data store is 
implemented to store, share, and process data. This store (e.g., AWS S3, Redis,
Azure Cloud Storage, GFS~\cite{2003-sosp-gfs}, Spanner~\cite{2012-osdi-spanner})
is a separate service from the compute, and is considered a ``tricky code'' that developers 
should ``avoid re-implementing''~\cite{2018-wsc-book}. More recently, there 
have also been a variety of runtime state storage services in the cloud like
Pocket for serverless~\cite{2018-osdi-pocket}, and Global Control Store in
Ray~\cite{2018-osdi-ray}. Put together, these external storage services in 
the cloud offer three primary advantages to edge applications: First, use of 
an external storage service decouples compute from data management, where 
developers can focus exclusively on the business- or application-logic without 
having to worry about if and how the data is stored. This decoupling also 
helps with reasoning about failures in a more principled manner (e.g., with 
serverless~\cite{2020-eurosys-ft-serverless}), which is one of the key challenges 
at the edge~\cite{2020-cacm-fail-edge}. Secondly, in such design advancements 
in a storage service (e.g., use of accelerated
hardware~\cite{2020-edgesys-keynote}, better compression or encoding 
algorithms~\cite{2019-hotedge-image-compression}) can be immediately used for the benefit of 
all edge applications. Lastly, a shared storage service allows for a better, 
consolidated management and utilization of storage resources, thus, enabling 
a more utility based edge computing model~\cite{2018-queue-edge-res}. Hence, 
we argue that having a first-class infrastructure storage service at the edge
would be beneficial to development and deployment of edge applications. 


We are clearly not the first one to make a case for an edge store
service~\cite{mortazavi2018pathstore,mayer2017fogstore}. However, prior 
work only addresses a subset of the edge storage requirements as we have 
shown in our previous work~\cite{griffin}. In this paper, we systematically 
analyze fundamental properties that have changed when moving from the cloud to the edge, 
and how these changes affect the design of a storage service for the edge 
(Section~\ref{sec:differences}). In Section~\ref{sec:programmability} we make 
a case for how programmable storage services can help to meet the requirements 
of edge applications.   




%Data here can be categorized into two types: application input and output data, 
%and runtime state. Input and output data represents large datasets 
%generated and processed in an edge deployment, such as streams of 
%videos, large-resolution images, and environment sensing data, etc. 
%State data on the other hand represents shared, collaborative runtime state 
%that an edge application might share between multiple endpoints. Examples 
%of shared state data can be ML/DL models, shared world state in AR/VR games, 
%aggregation states in analytics, and LiDAR data. Both of these datasets
%have different consistency, mobility, latency and persistency 
%requirements~\cite{2020-hotedge-griffin}. 


  
% The first approach to this research challenge is to redesign a new 
% storage service from scratch. With this goal in mind, a number of 
% storage systems is being investigated for edge computing 
% (like Pathstore and Fogstore \cite{mortazavi2018pathstore} \cite{mayer2017fogstore}). 
% These papers and prototypes provide insight into possible edge-based 
% storage services, but to the best of our knowledge they only address 
% a subset of the concerns (e.g. leaving out mobility) and do not 
% support any form of programmability that allows to tune the infrastructure 
% for the application's needs. Instead, we believe probrammability 
% is beneficial in a scenario where limited resources should be 
% used attentively, optimizing the resource utilization through 
% specialized rather than general-purpose operations, in order to harvest 
% the best performance for a diverse set of applications.
% 
% On the other side of the spectrum researchers are trying to 
% use existing cloud-native storage solutions at the edge. While using 
% these storage services might be beneficial due to their well-established 
% research and development efforts, adapting datacenter solutions like 
% Cassandra \cite{lakshman2010cassandra} does not come for free. 
% Due to the intrinsically different deployment of cloud datacenters 
% compared to edge computing, such storage solutions are catered 
% towards a different set of user requirements and infrastructure 
% assumptions. First of all, due to the different scale and distribution 
% of datacenters, there is no need to support mobility of users. 
% Adapting cloud storage services to the edge cannot prescind from 
% overcoming this in order to be feasible. In addition to the user 
% mobility requirement, another significant difference is that 
% storage services that were designed to operate in cloud datacenters 
% can generally operate under the assumptions of resource abundance 
% and reliability (e.g. elasticity and active infrastructure maintenance). 
% This is in sharp contrast with what happens in edge nodes, where 
% resources are limited and not transparently scalable. 
% 
% A storage service for edge computing cannot prescind from 
% providing support for user mobility, while at the same time 
% carefully managing resource allocation and usage in order to 
% allow different applications to coexist. As we will expand in 
% the next section, we believe that the difference between edge and 
% cloud deployment scenarios is vast and should be acknowledged by 
% the software solutions that run on top of it. We then 
% find ourselves in a convergence point. On the one hand, a 
% great variety of edge applications needs to use the infrastructure 
% to deliver low-latency responses. On the other hand, the 
% limited resource pool of edge nodes suggests that high-performance 
% datacenter solutions might not be feasible within the constraints. 
% In order to find a way out of this, we believe that the 
% target should be specialization and optimization of the infrastructure, 
% and we identify storage function programmability as a primary concern.

  

%While edge applications are diverse in their scope, it is possible to identify and categorize a subset of applications that are \textbf{stateful} and require data sharing in order to properly operate. Applications like collaborative machine learning, autonomous driving, video analytics, augmented reality and online edge games produce significant amounts of data and rely on the edge infrastructure for storage and processing. As it happens in cloud datacenters, the different applications are not homogeneous and rather might have different requirements in terms of consistency, mobility, latency and persistency of data. Given the complexity of the problem of combining limited edge resources and edge applications, research in the field is active but complex and it is exploring both existing cloud storage solutions and new, edge-native solutions. 

%The first approach to this research challenge is to redesign a new storage
% service from scratch. With this goal in mind, a number of storage systems is being investigated for edge computing (like Pathstore and Fogstore \cite{mortazavi2018pathstore} \cite{mayer2017fogstore}). These papers and prototypes provide insight into possible edge-based storage services, but to the best of our knowledge they only address a subset of the concerns (e.g. leaving out mobility) and do not support any form of programmability that allows to tune the infrastructure for the application's needs. Instead, we believe probrammability is beneficial in a scenario where limited resources should be used attentively, optimizing the resource utilization through specialized rather than general-purpose operations, in order to harvest the best performance for a diverse set of applications.

%On the other side of the spectrum researchers are trying to use existing
% cloud-native storage solutions at the edge. While using these storage services might be beneficial due to their well-established research and development efforts, adapting datacenter solutions like Cassandra \cite{lakshman2010cassandra} does not come for free. Due to the intrinsically different deployment of cloud datacenters compared to edge computing, such storage solutions are catered towards a different set of user requirements and infrastructure assumptions. First of all, due to the different scale and distribution of datacenters, there is no need to support mobility of users. Adapting cloud storage services to the edge cannot prescind from overcoming this in order to be feasible. In addition to the user mobility requirement, another significant difference is that storage services that were designed to operate in cloud datacenters can generally operate under the assumptions of resource abundance and reliability (e.g. elasticity and active infrastructure maintenance). This is in sharp contrast with what happens in edge nodes, where resources are limited and not transparently scalable.

%A storage service for edge computing cannot prescind from providing support for
% user mobility, while at the same time carefully managing resource allocation and usage in order to allow different applications to coexist. As we will expand in the next section, we believe that the difference between edge and cloud deployment scenarios is vast and should be acknowledged by the software solutions that run on top of it. We then find ourselves in a convergence point. On the one hand, a great variety of edge applications needs to use the infrastructure to deliver low-latency responses. On the other hand, the limited resource pool of edge nodes suggests that high-performance datacenter solutions might not be feasible within the constraints. In order to find a way out of this, we believe that the target should be specialization and optimization of the infrastructure, and we identify storage function programmability as a primary concern.

%In the next section we will highlight the infrastructural challenges that
% reinforce the case for programmability at the edge, and highlight the main differences from datacenter solutions that should be considered when designing a storage service for this landscape.

